Overcoming Data and Model Heterogeneities in Decentralized Federated Learning via Synthetic Anchors

Conventional Federated Learning (FL) involves collaborative training of a global model while maintaining user data privacy. One of its branches, decentralized FL, is a serverless network that allows clients to own and optimize different local models separately, which results in saving management and communication resources. Despite the promising advancements in decentralized FL, it may reduce model generalizability due to lacking a global model. In this scenario, managing data and model heterogeneity among clients becomes a crucial problem, which poses a unique challenge that must be overcome: How can every client's local model learn generalizable representation in a decentralized manner? To address this challenge, we propose a novel Decentralized FL technique by introducing Synthetic Anchors, dubbed as DeSA. Based on the theory of domain adaptation and Knowledge Distillation (KD), we theoretically and empirically show that synthesizing global anchors based on raw data distribution facilitates mutual knowledge transfer. We further design two effective regularization terms for local training: 1) REG loss that regularizes the distribution of the client's latent embedding with the anchors and 2) KD loss that enables clients to learn from others. Through extensive experiments on diverse client data distributions, we showcase the effectiveness of DeSA in enhancing both inter- and intra-domain accuracy of each client.

==> sections/04-theory.tex <==
\section{Theoretical Analysis on Generalization}\label{sec:theory}

\CY{maybe we need to remove i $\neq$ j}In this section, we focus on providing a theoretical justification for our proposed loss function and models.
Consider the $i$th client's local dataset $D_i$ which is sampled from the local data distribution $(\x,y)\sim P_i$. 
Taking the data heterogeneity into consideration, there exists at least two clients has different local data distributions, i.e. $\exists i\neq j$ s.t. $P_i \neq P_j$.
Also, denote the global data distribution as $P^T=\frac{1}{N}\sum_i P_i$ with the labeling function $f^T$: $y = f^T(\x)$, $\forall (\x,y)\sim P^T.$
Our ultimate goal is to have each client learn the local model $M_i$, which optimizes the global generalization error $\epsilon_{P^T}(M_i) = \mathbb{P}_{(\x,y)\sim P^T}[M_i(\x)\neq y]= \mathbb{P}_{(\x)\sim P^T}[M_i(\x)\neq f^T(\x)]$. We borrow the notion of $\mathcal{H} \Delta \mathcal{H}$ divergence from \cite{ben2010theory} that
    % $d_{\mathcal{H} \Delta \mathcal{H}}(D_s, D_T) =  \underset{h,h' \in \mathcal{H}}{\text{sup}} | \Pr_{x \sim D_s} (h(x) \neq h'(x)) - \Pr_{x \sim D_T} (h(x) \neq h'(x)) | $.
$d_{\mathcal{H} \Delta \mathcal{H}}(D_s, D_T) =  {\text{sup}}_{h,h' \in \mathcal{H}} | \Pr_{x \sim D_s} (h(x) \neq h'(x)) - \Pr_{x \sim D_T} (h(x) \neq h'(x)) | $.
We also define a constant $\lambda (P_i)$ for each client domain as $\lambda(P_i) = {\text{min}}_{M \in \mathcal{M}_i}  \epsilon_{P_T}(M) + \epsilon_{P_i} (M)$. 
%$\lambda(P_i) = \underset{M \in \mathcal{M}_i}{\text{min}} \ \  \epsilon_{P_T}(M) + \epsilon_{P_i} (M)$ }
Furthermore, we assume the global synthetic data $D^{Syn}$ are from the distribution $P^{Syn}$ with the corresponding labeling function $f^{Syn}$.
As $D^{Syn}$ is also leveraged for the knowledge distillation, inspired by \cite{feng2021kd3a}, we further denote the extended knowledge distillation (KD) dataset $D_{\text{KD}}^{Syn} = \{\x^{Syn}, \frac{1}{N-1}\sum_{i\neq j}M_j(\x^{Syn})\}\sim P_{\text{KD}}^{Syn}$, where $M_i(\x^{Syn})$ is the predicted logit on data $\x^{Syn}$ with the $i$th client's model. 
Obviously, $D_{\text{KD}}^{Syn}$ and $D^{Syn}$ shares the same distribution over $\x$, while the labeling function on $D_{\text{KD}}^{Syn}$ is $f_{\text{KD}}^{Syn}(\x) = \arg\max_c \frac{1}{N-1}\sum_{j\neq i} M_j(\x)$, where $c$ is the predicted class.
With the defined notation, the following theorem provides the global generalization bound for the $i$th client's model $M_i$.
\iffalse
\revision{Note that here `$P_s \rightarrow P_t$' refers to convergence in Probability}
\fi
\begin{thm}\label{Thm: general bound}
    Assume the model in $i$-th client $M_i=\rho_i \circ \psi_i$ from the model space $\mathcal{M}_i$. Let the training source data at $i$-th client compose of local data, synthetic data and extended KD data with the component weights $\boldsymbol{\alpha} = [\alpha, \alpha^{Syn},{\alpha}_{\text{KD}}^{Syn}]^\top$. If $\psi_i\circ P^{Syn}\rightarrow  \psi_i\circ P^T$  for any $\psi_i$, then the global generalization error can be bounded by
\begin{align}\label{Eq: general bound}
    \epsilon_{{P}^T}(M_i) \le &  \epsilon_{{P}_i^S}(M_i) + \frac{\alpha}{2} d_{\mathcal{H}\Delta\mathcal{H}}({P}_i ,{P}^{T}) + \alpha\lambda({P}_i)   \notag\\ & 
    + \alpha^{Syn} \epsilon_{{P}^T}(f^{Syn})  + \alpha^{Syn}_{\text{KD}} \epsilon_{{P}^T}(f_{\text{KD}}^{Syn}) .
\end{align}
\end{thm}
% \begin{align}
%     \alpha = |D_i|/(1+\lambda_{\text{KD}})(|D_i|+|D^{syn}|)\\
%     \alpha^{syn} = |D_{syn}|/(1+\lambda_{\text{KD}})(|D_i|+|D^{syn}|)\\
%     \alpha^{syn}_{\text{KD}} = \lambda_{\text{KD}})/(1+\lambda_{\text{KD}})\\
% \end{align}




% From Eq.~(\ref{Eq: general bound}), it can be seen that the generalization bound for $M_i$ consists of five terms: The first term $\epsilon_{{P}_i^S}(h)$ is the error bound with respect to the training source data distribution. With Claim~\ref{Claim: equivalent} in appendix, minimizing this term is equivalent to optimizing the loss $\alpha \mathbb{E}_{(\x,y)\sim P_i}\mathcal{L}_{\text{CE}} + \alpha^{Syn} \mathbb{E}_{(\x,y)\sim P^{Syn}}\mathcal{L}_{\text{CE}} + \alpha^{Syn}_{\text{KD}}\mathbb{E}_{(\x,y)\sim P^{Syn}}L_{\text{KD}}$.  
% \footnote{Note that the empirical implementation~(\ref{glob}) has $\alpha\propto |D_i|/(1+\lambda_{\text{KD}})(|D_i|+|D^{{Syn}}|)$, 
% $\alpha^{Syn}\propto |D^{Syn}|/(1+\lambda_{\text{KD}})(|D_i|+|D^{{Syn}}|)$, 
% $\alpha^{Syn}_{KD}\propto \lambda_{\text{KD}}/(1+\lambda_{\text{KD}})$. Thus, we can adjust the component weights by the size of synthetic data and regularization hyperparameter.}

% The fourth term is to measure the discrepancy between real labeling and the synthetic data labeling mechanisms.
% As the gap of the two labeling mechanisms is close, we will have small term.
% The fifth term is from the knowledge distillation loss, in which we use the consensus knowledge to improve the local model. 
% As the consensus knowledge is close to the true labeling function, this term will be negligible.
We provide the interpretation for Theorem~\ref{Thm: general bound} in Appendix~\ref{Thm:interpretation}. Furthermore, the following proposition implies our generalization bound in Theorem~\ref{Thm: general bound} is tighter than the original bound under some mild conditions. 
\begin{prop}\label{Prop: tighter bound}
Under the conditions in Theorem~\ref{Thm: general bound}, if it further holds that 
\begin{align}\label{Eq: tighter bound}
\sup_{M\in\mathcal{M}_i} \min \{ &|\epsilon_{P^{Syn}}(M) -  \epsilon_{{P}^T}(M)| +   \epsilon_{{P}^T}(f^{Syn}), 
\notag \\ & |\epsilon_{P_{\text{KD}}^{Syn}}(M) - \epsilon_{{P}^T}(M)| + \epsilon_{{P}^T}(f_{\text{KD}}^{Syn}) \}  
\notag \\ & \le \inf_{M\in\mathcal{M}_i}|\epsilon_{P_i}(M) - \epsilon_{{P}^T}(M)| 
\notag \\ &+ \frac{1}{2} d_{\mathcal{M}_i\Delta\mathcal{M}_i}({P}_i ,{P}^{T}) + \lambda({P}_i),
\end{align}
then we can get a tighter generalization bound on the $i$th client's model $M_i$ than local learning.
%than just learning with its local data. 
\vspace{-2mm}
\end{prop}
When the local data heterogeneity is severe,  $\inf_{M\in\mathcal{M}_i}|\epsilon_{P_i}(M) - \epsilon_{{P}^T}(M)|$ and $d_{\mathcal{M}_i\Delta\mathcal{M}_i}({P}_i ,{P}^{T})$ would be large.
As the synthetic data and the extended KD data are approaching the the global data distribution, the left side term in (\ref{Eq: tighter bound}) would be small.
Thus, the above proposition points out that, to reach better generalization, the model learning should rely more on the synthetic data and the extended KD data, when the local data are highly heterogeneous and the synthetic and the extended KD datasets are similar to the global ones.




==> sections/table2_intra_inter.tex <==
\begin{table*}[t]
\centering
\caption{\small \CY{change to global acc}Heterogeneous model experiments. We compare with baseline FL methods that can handle both data and model heterogeneity on the intra and inter-client test accuracy$^{\small a}$.}
\label{tab:hetero_model}
%\resizebox{\linewidth}{!}{
\begin{adjustbox}{max width=\textwidth}
\begin{threeparttable}
\begin{tabular}{lll|llllll|lllll|ll}
\toprule
\multicolumn{3}{l|}{\multirow{2}{*}{}}                                                        & \multicolumn{6}{l|}{\texttt{DIGITS}}                                                                                                                             & \multicolumn{5}{l|}{\texttt{OFFICE}}                                                                                               & \multicolumn{2}{l}{\texttt{CIFAR10C}}       \\ \cline{4-16} 
\multicolumn{3}{l|}{}                                                                         & \multicolumn{1}{l|}{MN(C)\tnote{b}} & \multicolumn{1}{l|}{SV(A)} & \multicolumn{1}{l|}{US(C)} & \multicolumn{1}{l|}{Syn(A)} & \multicolumn{1}{l|}{MM(C)} & Avg   & \multicolumn{1}{l|}{AM(A)} & \multicolumn{1}{l|}{CA(C)} & \multicolumn{1}{l|}{DS(A)} & \multicolumn{1}{l|}{WE(A)} & Avg   & \multicolumn{1}{l|}{0.1}   & 0.2\\ \hline
\multicolumn{2}{l|}{\multirow{2}{*}{Standalone}}                                           & intra & \multicolumn{1}{l|}{98.96} & \multicolumn{1}{l|}{85.64} & \multicolumn{1}{l|}{\textbf{98.76}} & \multicolumn{1}{l|}{94.70}  & \multicolumn{1}{l|}{94.61} & 94.53 & \multicolumn{1}{l|}{70.31} & \multicolumn{1}{l|}{57.78} & \multicolumn{1}{l|}{71.88} & \multicolumn{1}{l|}{89.83} & 72.45 & \multicolumn{2}{c}{65.75} \\ \cline{3-3}
\multicolumn{2}{l|}{}                                                                 & inter & \multicolumn{1}{l|}{52.24} & \multicolumn{1}{l|}{61.68} & \multicolumn{1}{l|}{41.37} & \multicolumn{1}{l|}{72.67}  & \multicolumn{1}{l|}{69.48} & 60.69 & \multicolumn{1}{l|}{24.85} & \multicolumn{1}{l|}{46.42} & \multicolumn{1}{l|}{22.93} & \multicolumn{1}{l|}{39.06} & 33.34 & \multicolumn{2}{c}{53.76} \\ \hline
\multicolumn{2}{l|}{\multirow{2}{*}{FedHe}}                                           & intra & \multicolumn{1}{l|}{98.89} & \multicolumn{1}{l|}{83.33} & \multicolumn{1}{l|}{\textbf{98.76}} & \multicolumn{1}{l|}{93.89}  & \multicolumn{1}{l|}{94.31} & 93.84 & \multicolumn{1}{l|}{72.40} & \multicolumn{1}{l|}{55.56} & \multicolumn{1}{l|}{71.88} & \multicolumn{1}{l|}{91.53} & 72.84 & \multicolumn{1}{l|}{60.10} & 63.77 \\ \cline{3-3}
\multicolumn{2}{l|}{}                                                                 & inter & \multicolumn{1}{l|}{49.67} & \multicolumn{1}{l|}{62.50} & \multicolumn{1}{l|}{37.67} & \multicolumn{1}{l|}{70.77}  & \multicolumn{1}{l|}{65.89} & 57.30 & \multicolumn{1}{l|}{20.31} & \multicolumn{1}{l|}{44.37} & \multicolumn{1}{l|}{25.19} & \multicolumn{1}{l|}{40.10} & 32.50 & \multicolumn{1}{l|}{42.36} & 47.83 \\ \hline
\multicolumn{1}{l|}{\multirow{4}{*}{FedDF}} & \multicolumn{1}{l|}{\multirow{2}{*}{Cifar100}} & intra & \multicolumn{1}{l|}{98.81}      & \multicolumn{1}{l|}{82.47}      & \multicolumn{1}{l|}{98.76}      & \multicolumn{1}{l|}{92.51}       & \multicolumn{1}{l|}{94.72}      &  93.45   & \multicolumn{1}{l|}{63.54} & \multicolumn{1}{l|}{50.22} & \multicolumn{1}{l|}{43.75} & \multicolumn{1}{l|}{79.66} & 59.29 & \multicolumn{1}{l|}{48.46} & 59.98 \\ \cline{3-3}
\multicolumn{1}{l|}{}                       & \multicolumn{1}{l|}{}                   & inter & \multicolumn{1}{l|}{57.77}      & \multicolumn{1}{l|}{60.90}      & \multicolumn{1}{l|}{51.93}      & \multicolumn{1}{l|}{63.94}       & \multicolumn{1}{l|}{69.42}      &   60.79    & \multicolumn{1}{l|}{30.64} & \multicolumn{1}{l|}{49.28} & \multicolumn{1}{l|}{29.57} & \multicolumn{1}{l|}{35.96} & 36.36 & \multicolumn{1}{l|}{34.90} & 41.87 \\ \cline{2-16} 
\multicolumn{1}{l|}{}                       & \multicolumn{1}{l|}{\multirow{2}{*}{FMNIST}} & intra & \multicolumn{1}{l|}{98.71} & \multicolumn{1}{l|}{85.25} & \multicolumn{1}{l|}{98.92} & \multicolumn{1}{l|}{93.54}  & \multicolumn{1}{l|}{94.08} & 94.10 & \multicolumn{1}{l|}{67.71} & \multicolumn{1}{l|}{55.46} & \multicolumn{1}{l|}{69.75}  & \multicolumn{1}{l|}{76.27} & 67.07 & \multicolumn{1}{l|}{38.52} & 47.24 \\ \cline{3-3}
\multicolumn{1}{l|}{}                       & \multicolumn{1}{l|}{}                   & inter & \multicolumn{1}{l|}{29.14} & \multicolumn{1}{l|}{65.11} & \multicolumn{1}{l|}{31.46} & \multicolumn{1}{l|}{69.95}  & \multicolumn{1}{l|}{65.57} & 52.24 & \multicolumn{1}{l|}{29.60}  & \multicolumn{1}{l|}{43.55} & \multicolumn{1}{l|}{30.39} & \multicolumn{1}{l|}{32.94} & 34.12 & \multicolumn{1}{l|}{21.37} & 27.33\\ \hline
\multicolumn{1}{l|}{\multirow{4}{*}{FCCL}}  & \multicolumn{1}{l|}{\multirow{2}{*}{Cifar100}} & intra & \multicolumn{1}{l|}{11.25}      & \multicolumn{1}{l|}{19.10}      & \multicolumn{1}{l|}{13.66}      & \multicolumn{1}{l|}{10.08}       & \multicolumn{1}{l|}{11.25}      &  13.07     & \multicolumn{1}{l|}{64.06} & \multicolumn{1}{l|}{50.67} & \multicolumn{1}{l|}{62.50} & \multicolumn{1}{l|}{84.75} & 65.50 & \multicolumn{1}{l|}{\textbf{63.10}} & \textbf{65.33} \\ \cline{3-3}
\multicolumn{1}{l|}{}                       & \multicolumn{1}{l|}{}                   & inter & \multicolumn{1}{l|}{13.52}      & \multicolumn{1}{l|}{11.56}      & \multicolumn{1}{l|}{12.92}      & \multicolumn{1}{l|}{13.82}       & \multicolumn{1}{l|}{13.52}      &    13.07   & \multicolumn{1}{l|}{29.60} & \multicolumn{1}{l|}{48.58} & \multicolumn{1}{l|}{38.74} & \multicolumn{1}{l|}{41.43} & 39.59 & \multicolumn{1}{l|}{\textbf{51.68}} & \textbf{53.73} \\ \cline{2-16} 
\multicolumn{1}{l|}{}                       & \multicolumn{1}{l|}{\multirow{2}{*}{FMNIST}} & intra & \multicolumn{1}{l|}{95.01} & \multicolumn{1}{l|}{72.92} & \multicolumn{1}{l|}{94.73} & \multicolumn{1}{l|}{86.11}  & \multicolumn{1}{l|}{90.10} & 87.78 & \multicolumn{1}{l|}{67.19} & \multicolumn{1}{l|}{54.67} & \multicolumn{1}{l|}{68.75} & \multicolumn{1}{l|}{86.44} & 69.26 & \multicolumn{1}{l|}{13.51} & 13.51 \\ \cline{3-3}
\multicolumn{1}{l|}{}                       & \multicolumn{1}{l|}{}                   & inter & \multicolumn{1}{l|}{34.29} & \multicolumn{1}{l|}{58.04} & \multicolumn{1}{l|}{29.62} & \multicolumn{1}{l|}{57.28}  & \multicolumn{1}{l|}{60.46} & 47.94 & \multicolumn{1}{l|}{14.12} & \multicolumn{1}{l|}{44.15} & \multicolumn{1}{l|}{28.50} & \multicolumn{1}{l|}{35.81} & 30.65 & \multicolumn{1}{l|}{12.48} & 12.48 \\ \hline
\multicolumn{2}{l|}{\multirow{2}{*}{FedProto}}                                           & intra & \multicolumn{1}{l|}{98.41} & \multicolumn{1}{l|}{88.52} & \multicolumn{1}{l|}{97.85} & \multicolumn{1}{l|}{96.92}  & \multicolumn{1}{l|}{93.62} & 95.04 & \multicolumn{1}{l|}{69.79} & \multicolumn{1}{l|}{36.44} & \multicolumn{1}{l|}{53.13} & \multicolumn{1}{l|}{88.14} & 61.86 & \multicolumn{1}{l|}{16.27} & 23.05\\ \cline{3-3}
\multicolumn{2}{l|}{}                                                                 & inter & \multicolumn{1}{l|}{53.64} & \multicolumn{1}{l|}{67.55} & \multicolumn{1}{l|}{48.69} & \multicolumn{1}{l|}{77.26}  & \multicolumn{1}{l|}{\textbf{69.64}} & 63.36 & \multicolumn{1}{l|}{27.51} & \multicolumn{1}{l|}{21.27} & \multicolumn{1}{l|}{17.61} & \multicolumn{1}{l|}{33.58} & 24.99 & \multicolumn{1}{l|}{15.63} & 19.35\\ \hline
\multicolumn{2}{l|}{\multirow{2}{*}{\ours{}($D_{\rm VHL}^{Syn}$)\tnote{d}}}                                       & intra & \multicolumn{1}{l|}{98.69} & \multicolumn{1}{l|}{80.09} & \multicolumn{1}{l|}{98.66} & \multicolumn{1}{l|}{90.68}  & \multicolumn{1}{l|}{94.40} & 92.50 & \multicolumn{1}{l|}{10.42} & \multicolumn{1}{l|}{57.33} & \multicolumn{1}{l|}{28.13} & \multicolumn{1}{l|}{89.83} & 46.43 & \multicolumn{1}{l|}{47.99} & 54.42 \\ \cline{3-3}
\multicolumn{2}{l|}{}                                                                 & inter & \multicolumn{1}{l|}{43.33} & \multicolumn{1}{l|}{57.51} & \multicolumn{1}{l|}{28.26} & \multicolumn{1}{l|}{62.02}  & \multicolumn{1}{l|}{67.69} & 51.76 & \multicolumn{1}{l|}{8.28}  & \multicolumn{1}{l|}{46.20} & \multicolumn{1}{l|}{13.16} & \multicolumn{1}{l|}{35.56} & 25.80 & \multicolumn{1}{l|}{28.18} & 34.86 \\ \hline
\multicolumn{2}{l|}{\multirow{2}{*}{\ours{}}}                                            & intra & \multicolumn{1}{l|}{\textbf{99.04}} & \multicolumn{1}{l|}{\textbf{87.90}} & \multicolumn{1}{l|}{98.71} & \multicolumn{1}{l|}{\textbf{97.00}}  & \multicolumn{1}{l|}{\textbf{94.98}} & \textbf{95.52} & \multicolumn{1}{l|}{\textbf{78.65}} & \multicolumn{1}{l|}{61.78} & \multicolumn{1}{l|}{53.13} & \multicolumn{1}{l|}{\textbf{91.53}} & \textbf{71.27} & \multicolumn{1}{l|}{59.87} & 63.68 \\ \cline{3-3}
\multicolumn{2}{l|}{}                                                                 & inter & \multicolumn{1}{l|}{\textbf{62.89}} & \multicolumn{1}{l|}{\textbf{73.24}} & \multicolumn{1}{l|}{\textbf{64.29}} & \multicolumn{1}{l|}{\textbf{77.13}}  & \multicolumn{1}{l|}{68.54} & \textbf{69.21} & \multicolumn{1}{l|}{\textbf{49.09}} & \multicolumn{1}{l|}{\textbf{53.67}} & \multicolumn{1}{l|}{\textbf{24.67}} & \multicolumn{1}{l|}{\textbf{44.26}} & \textbf{42.92} & \multicolumn{1}{l|}{42.70} & 49.20 \\ \bottomrule
\end{tabular}
\begin{tablenotes}
    \item[a] Intra and inter-client test accuracy are defined as  testing $i$-th local model on client $i$'s test set and every client $j$'s ($\forall j \neq i, j \in [N]$) test sets, respectively. 
    \item[b] The letter inside the parenthesis is the model architecture used by the client. A and C represent AlexNet and ConvNet, respectively. 
    \item[c] The best accuracy is marked in \textbf{bold}.
    \item[d] For VHL baseline, we use the synthetic data sampling strategy in VHL only. The purpose is to show \ours{} can generate better synthetic anchor data for feature regularization and knowledge distillation.
\end{tablenotes}
\end{threeparttable}
\end{adjustbox}
%
\vspace{-5mm}
\end{table*}
